Reach-Avoid Problems via Sum-of-Squares Optimization and Dynamic Programming

Reach-avoid problems involve driving a system to a set of desirable configurations while keeping it away from undesirable ones. Providing mathematical guarantees for such scenarios is challenging but have numerous potential practical applications. Due to the challenges, analysis of reach-avoid problems involves making trade-offs between generality of system dynamics, generality of problem setups, optimality of solutions, and computational complexity. In this paper, we combine sum-of-squares optimization and dynamic programming to address the reach-avoid problem, and provide a conservative solution that maintains reaching and avoidance guarantees. Our method is applicable to polynomial system dynamics and to general problem setups, and is more computationally scalable than previous related methods. Through a numerical example involving two single integrators, we validate our proposed theory and compare our method to Hamilton-Jacobi reachability. Having validated our theory, we demonstrate the computational scalability of our method by computing the reach-avoid set of a system involving two kinematic cars.

==> def.tex <==
%% !TEX root = main.tex
\section{Definitions}\label{sec:def}




==> notes.tex <==
%% !TEX root = main.tex
\section{Notes and to do \label{sec:notes}}

To do for this paper:
\begin{enumerate}
  \item Write out the indicator function formulation for the objective function, probably in Section \ref{sec:sos}.
  \item Do at least one numerical simulation. If only one type of simulation can be done, probably do two closed-loop simulations. Should we compare with HJI? If so, ask for Scott's help. (Probably wait for journal version on this)
  \item Revise SOS background to make everything in terms of state, not time.
  \item Write up any numerical details (eg. initialization of sets) in subsection \ref{subsec:imp}.
  \item Write up simulations section
  \item Write conclusions
\end{enumerate}

Futuer work:
\begin{itemize}
  \item For the open-loop case, we can use Joe's results. This could be a separate conference paper, and be included in a journal paper.
  \item For the closed-loop case, we can compare with HJI, maybe using what Scott has done. This could be for a journal paper
\end{itemize}

Other notes:
\begin{itemize}
  \item If control saturation is too much of a pain, try the other formulation in Section IV-B of A. Majumdar, A. A. Ahmadi, and R. Tedrake, “Control design along trajectories with sums of squares programming,” in 2013 IEEE International Conference on Robotics and Automation, 2013, pp. 4054–4061.
  \item What would be good applications for differential games? Perhaps car overtaking bicycle
\end{itemize}
